Multiparty testing preorders

Variants of the must testing approach have been successfully applied in service oriented computing for analysing the compliance between (contracts exposed by) clients and servers or, more generally, between two peers. It has however been argued that multiparty scenarios call for more permissive notions of compliance because partners usually do not have full coordination capabilities. We propose two new testing preorders, which are obtained by restricting the set of potential observers. For the first preorder, called uncoordinated, we allow only sets of parallel observers that use different parts of the interface of a given service and have no possibility of intercommunication. For the second preorder, that we call individualistic, we instead rely on parallel observers that perceive as silent all the actions that are not in the interface of interest. We have that the uncoordinated preorder is coarser than the classical must testing preorder and finer than the individualistic one. We also provide a characterisation in terms of decorated traces for both preorders: the uncoordinated preorder is defined in terms of must-sets and Mazurkiewicz traces while the individualistic one is described in terms of classes of filtered traces that only contain designated visible actions and must-sets.

==> related.tex <==

Several variants of the must testing preorder, contract compliance and
sub-contract relation have been developed in the literature to deal with
several aspects of services compositions, such as buffered asynchronous
communication
~\cite{bravetti2008foundational,padovani2010contract,mostrous2009global},
fairness~\cite{padovani2011fair},
peer-interaction~\cite{bernardi2013mutually}, among others. We remark that
these approaches deal with aspects that are orthogonal to the discriminating
power of the distributed tests analysed in this work. There are some
similarities with approaches dealing with buffered communications due to the
fact that actions may be reordered. Nevertheless, our work addresses a
synchronous communication model and, hence, message reordering is not related
to the possibility of reordering buffered messages; we left the study of
distributed tests under asynchronous communication as a future work. We still
remark that, even in presence of the reordering of actions, the preorders
proposed in this paper are different from the ones
in~\cite{bravetti2008foundational,padovani2010contract,mostrous2009global}.
The paradigmatic examples are $ \tau.\co{a} + \tau.\co{b}
\dmustleq{{\{a\},\{b\}}} 0$ and $a.c + b.d \lmusteq{\{a,b\},\{c,d\}} a.d +
b.c$, which do not hold for any of the preorders with buffered communication.
The main reason is that in presence of asynchronous communication the test
$a.\one + b.\one$ distinguishes $ \tau.\co{a} + \tau.\co{b}$ from $0$ and
$\one + \co{a}.(\one + \co{d}.\zero)$ distinguishes $a.c+b.d$ from $a.d+b.c$.
These clients, however, do not represent a set of \distributed\ partners
without runtime communication. To the best of our knowledge the only attempt
to deal with multi-agent testing have been suggested
in~\cite{hennessyWS25CCC}, but the development of the theory has been left as
future work.

